Duwak: Dual Watermarks in Large Language Models

As large language models (LLM) are increasingly used for text generation tasks, it is critical to audit their usages, govern their applications, and mitigate their potential harms. Existing watermark techniques are shown effective in embedding single human-imperceptible and machine-detectable patterns without significantly affecting generated text quality and semantics. However, the efficiency in detecting watermarks, i.e., the minimum number of tokens required to assert detection with significance and robustness against post-editing, is still debatable. In this paper, we propose, Duwak, to fundamentally enhance the efficiency and quality of watermarking by embedding dual secret patterns in both token probability distribution and sampling schemes. To mitigate expression degradation caused by biasing toward certain tokens, we design a contrastive search to watermark the sampling scheme, which minimizes the token repetition and enhances the diversity. We theoretically explain the interdependency of the two watermarks within Duwak. We evaluate Duwak extensively on Llama2 under various post-editing attacks, against four state-of-the-art watermarking techniques and combinations of them. Our results show that Duwak marked text achieves the highest watermarked text quality at the lowest required token count for detection, up to 70% tokens less than existing approaches, especially under post paraphrasing.

==> generations.tex <==
\begin{tabular}{llll}
\toprule
 &  &  & response \\
prompt & generator & delta &  \\
\midrule
\multirow[t]{11}{*}{[INST] <<SYS>> You are a helpful assistant. Always answer in the most accurate way. <</SYS>> Write a story about a retired astronaut that joins a risky interstellar rescue mission.. [/INST]} & BINARY & 1.500000 &   John "Hawk" Hawkins had seen it all during his illustrious career as an astronaut. He had flown on dozens of missions to space, including the historic first manned voyage to Mars, and had even broken a record for the longest time spent in space. But after decades of flying through the cosmos, Hawk decided it was time to hang up his space suit and enjoy his well-deserved retirement.___LINE______LINE___That was until he received a distress call from a nearby planet that had been devastated by a catastrophic event \\
\cline{2-4}
 & CS & 2.500000 &  Title: The Call of Duty___LINE______LINE___Retired astronaut John "Hawk" Hawkins had seen it all during his illustrious career in space exploration. From the vastness of the cosmos to the intricate workings of the human body, he had experienced it all. But at the age of 65, he thought he had left his adventurous days behind \\
\cline{2-4}
 & CS+EXP & 2.500000 &  Title: The Call of Duty___LINE______LINE___John "Hawk" Hawkins, a retired astronaut in his early sixties, had grown accustomed to the quiet life on Earth. After decades of space travel, he had left the thrill of exploration behind and settled into a comfortable routine. However, fate had other plans.___LINE______LINE___One fateful evening, while watching the news, Hawk's eyes widened as he listened to the urgent message from Mission Control: an interstellar rescue mission was underway, and they needed his expertise \\
\cline{2-4}
 & \multirow[t]{2}{*}{CS+KGW} & 2.500000 &  Title: The Call of Duty___LINE______LINE___Retired astronaut John "Jack" Jackson had spent his entire adult life working for NASA, logging over a hundred days in space and earning a reputation as one of the best pilots in the business. But after a near-fatal accident on a mission to Mars, he was forced to retire and leave his beloved space travel behind.___LINE______LINE___Years went by, and Jack found himself growing restless and unfulfilled in his post-NASA life. He spent his days golfing and fishing, but something was missing \\
 &  & 3.000000 &  Title: The Call of Duty___LINE______LINE___Dr. Emma Taylor, a retired astronaut in her early fifties, lived a quiet life in a small town near NASA's Johnson Space Center in Houston, Texas. After decades of dedicating herself to space exploration, Emma had decided to hang up her space suit for good, content with her achievements and the memories of her time in space \\
\cline{2-4}
 & EXP & 1.500000 &   Title: The Courageous Retiree___LINE______LINE___John "Hawk" Hawkins, a grizzled astronaut in his early sixties, had long since left his spacefaring days behind. Or so he thought. When he received the phone call from Mission Control, his heart raced with a mixture of excitement and trepidation \\
\cline{2-4}
 & \multirow[t]{5}{*}{KGW} & 1.500000 &   Title: The Cosmic Call___LINE______LINE___Dr. Emma Taylor had seen it all during her illustrious career as an astronaut. From the depths of space to the farthest reaches of the cosmos, she had explored it all \\
 &  & 2.000000 &   Title: The Call of Duty___LINE______LINE___Dr. Emma Taylor had seen it all during her illustrious career as an astronaut. From the vastness of space to the intricate workings of the human body, she had explored it all \\
 &  & 2.500000 &   Title: The Call of Duty___LINE______LINE___Mission Briefing:___LINE______LINE___Mission Objective: Retrieve the last surviving member of the Icarus Expedition, stranded on a hostile exoplanet.___LINE______LINE___Mission Location: Planet Xylophia-IV, located 4.5 light years from Earth.___LINE______LINE___Mission Profile: The Icarus Expedition was sent to explore Xylophia-IV over 5 years ago. Upon reaching the planet's atmosphere, their spacecraft encountered unexpected storms and malfunctions, causing them to crash-land on the hostile surface. The surviving member of the expedition, Captain Emma Taylor, has been stranded on the planet for over 4 years, with limited supplies and medical equipment \\
 &  & 3.000000 &   Title: The Call of Duty___LINE______LINE___Dr. Emma Taylor had seen it all during her illustrious career as an astronaut. From the vastness of space to the tiniest details of spacecraft engineering, she had devoted herself to advancing humanity's understanding of the cosmos \\
 &  & 3.500000 &   Title: The Call of Duty___LINE______LINE___Dr. Emma Grey had seen it all during her illustrious career as an astronaut. From the euphoric heights of spacewalks to the terrifying lows of spacecraft malfunctions, Emma had experienced it all \\
\cline{1-4} \cline{2-4}
\bottomrule
\end{tabular}




==> proof.tex <==
\section*{Proofs}
\setcounter{section}{3}

\begin{definition}[Spike Entropy]
Given a discrete probability vector \(p\) and a scalar \(z\), the spike entropy of \(p\) with respect to \(z\) is defined as
\[
S(p, z) = \sum^n \frac{p^n}{1 + z p^n}.
\]
\end{definition}


\begin{theorem}[Green List Tokens in \algo]
Consider a set of text sequences, each with \(T\) tokens, generated from a language model. These sequences are sampled by a base probability vector \(p_{t}\) for each token $x_{t}$. In this process, a random selection of green list tokens, constituting \(\gamma N\) of the total, is elevated in priority by incrementing their logits by \(\delta\). Define \(\beta\) as \(\exp(\delta)\) and \(|x|_{\mathcal{G}}\) as the frequency of green list tokens within a sequence \(x\). If a selection of the top-k tokens is based on the revised probabilities, and the final token is randomly chosen from these top candidates. The established bounds in KGW for expected green list token number and their variance are still hold.
\end{theorem}

\begin{proof}
Specifically,
For a sequence marked by watermarks, possessing an average spike entropy no less than \(S^{\star}\), that is,
\[
\frac{1}{T} \sum_t S\left(p_{t}, \frac{(1-\gamma)(\beta-1)}{1+(\beta-1) \gamma}\right) \geq S^{\star},
\]
the minimum expected count of green list tokens in the sequence is
\[
\mathbb{E}|x|_G \geq \frac{\gamma \beta T}{1+(\beta-1) \gamma} S^{\star}.
\]
Furthermore, the variance in the count of these green list tokens is limited to
\[
\operatorname{Var}|x|_{\mathcal{G}} \leq T \frac{\gamma \beta S^{\star}}{1+(\beta-1) \gamma}\left(1-\frac{\gamma \beta S^{\star}}{1+(\beta-1) \gamma}\right),
\]
Referencing Lemma E.1 from \cite{kirchenbauer2023watermark}, when a token index \(k\) is sampled from the watermarked distribution, the probability that the token is from the green list is at least
\begin{equation}
\mathbb{P}[k \in G] \geq \frac{\gamma \alpha}{1+(\alpha-1) \gamma} S\left(p, \frac{(1-\gamma)(\alpha-1)}{1+(\alpha-1) \gamma}\right).
\end{equation}
In the context of approximate top-k sampling, where we independently sample \(K\) words from the vocabulary, the number of words sampled from the green list in the top-k selection approximates \(K \times \mathbb{P}[k \in \mathcal{G}]\). Given the large vocabulary set, this approximation holds. Therefore, the final sampled token from the green list is also approximately \(\mathbb{P}[k \in \mathcal{G}]\). Thus, Theorem 4.2 from \cite{kirchenbauer2023watermark} is applicable in our modified sampling method.

\end{proof}


\begin{theorem}[Perplexity in Enhanced Watermark]
    Consider a language model that produces a probability vector \( p_{t} \) for the token at position \( T \). When this model is modified with a watermark, it predicts tokens using an altered probability vector \( \hat{p}_{t} \). Let \( \mathcal{V}_{\text{top-k}} \) denote the set of top \( k \) tokens with the highest probabilities in \( \hat{p}_{t} \). The modified probability vector after top-k sampling is denoted as \( \hat{p}^{'}_{t} \). Under top-k sampling, the expected perplexity of the \( T \)th token, with respect to the randomness of the partition into `green' and `red' lists, is bounded above by a factor of the original model's perplexity, scaled by \( \beta \), i.e.,
    \[
    -\underset{\mathcal{G}, \mathcal{R}}{\mathbb{E}} \sum_n \hat{p}^{'n}_{t} \ln \left(p^n_{t}\right) \leq \beta P^*
    \]
    where \( P^* = -\sum_n p^n_{t} \ln \left(p^n_{t}\right) \) is the perplexity of the original model.
\end{theorem}

\begin{proof}
    
% \subsection*{Proof}

Given the top-k sampling, the normalized probability for a token $n$ in $V_{top-k}$ is:
\begin{equation}
    \hat{p}^{'n} = \frac{p^n}{\sum_{i \in \mathcal{V}_{top-k}} p^i}.
\end{equation}

The expectation of the modified probability distribution, considering the partition into the green list $\mathcal{G}$ and the red list $\mathcal{R}$, is decomposed as follows:
\begin{itemize}
    \item For $n$ in $\mathcal{G} \cap \mathcal{V}_{top-k}$, the normalized probability is amplified by a factor $\beta$:
    % \begin{equation}
    %     \underset{\mathcal{G}, \mathcal{R}, n \in \mathcal{G} \cap V_{top-k}}{\mathbb{E}} \frac{\beta \hat{p}^{'n}}{\sum_{i \in R \cap \mathcal{V}_{top-k}} \hat{p}^{'i} + \beta \sum_{i \in \mathcal{G} \cap V_{top-k}} \hat{p}^{'i}}.
    % \end{equation}
    %\je{Alternative using selector function}
    \begin{equation}
        \underset{\mathcal{G}, \mathcal{R}, n \in \mathcal{G} \cap V_{top-k}}{\mathbb{E}} \frac{\beta \hat{p}^{'n}}{\sum_{i \in \mathcal{V}_{top-k}} \beta^{\mathbbm{1}[i\in \mathcal{G}]}\hat{p}^{'i}}.
    \end{equation}
    \item For $n$ in $\mathcal{R} \cap \mathcal{V}_{top-k}$, the probability remains as $\hat{p}^{'n}$, thus the expectation becomes:
    % \begin{equation}
    %     \underset{\mathcal{G}, \mathcal{R}, n \in R \cap V_{top-k}}{\mathbb{E}} \frac{\hat{p}^{'n}}{\sum_{i \in \mathcal{R} \cap \mathcal{V}_{top-k}} \hat{p}^{'i} + \beta \sum_{i \in \mathcal{G} \cap \mathcal{V}_{top-k}} \hat{p}^{'i}}.
    % \end{equation}
    %\je{Alternative using selector function}
    \begin{equation}
        \underset{\mathcal{G}, \mathcal{R}, n \in R \cap \mathcal{V}_{top-k}}{\mathbb{E}} \frac{\hat{p}^{'n}}{\sum_{i \in \mathcal{V}_{top-k}} \beta^{\mathbbm{1}[i\in\mathcal{G}]} \hat{p}^{'i}}.
    \end{equation}
\end{itemize}

The general inequality for any $n \in \mathcal{V}_{top-k}$ is:
\begin{equation}
    \underset{\mathcal{G}, \mathcal{R}}{\mathbb{E}} \big[ \hat{p}^n \big] \leq (1 + (\beta - 1) \gamma_{top-k}) \hat{p}^{'n}.
\end{equation}
where $\gamma_{top-k}$ is the portion of green list token selected by top-k sampling.

The final expected perplexity for the model under these conditions is:
\begin{equation}
   -\underset{\mathcal{G}, \mathcal{R}}{\mathbb{E}} \sum_n \hat{p}_t^{\prime n} \ln \left(p_t^n\right) \leq (1 + (\beta - 1) \gamma_{top-k}) P^*_{top-k} \leq \beta P^*_{top-k}\leq \beta P^*,
\end{equation}
where $P^*_{top-k}$ represents the original top-k perplexity of the model.
\end{proof}


==> tables.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison of watermarking methods on different metrics. Arrows indicate the direction of better performance: a downward arrow (\(\downarrow\)) means lower values are better, and an upward arrow (\(\uparrow\)) means higher values are better.}
\label{tab:watermark_comparison}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
Watermark     & Human Text & No Watermark & KGW & EXP & BINARY & ITS & CS & KGW+EXP & CS+EXP & CS+KGW \\ 
\midrule
Diversity\% (\(\uparrow\))  & 93.62 & 86.66 & 81.41 & 39.58 & 44.56 & 78.72 & 86.53 & 17.9 & 83.98 & 83.83 \\
MAUVE\% (\(\uparrow\))      & 100   & 82.36 & 75.5  & 55.87 & 55.57 & 79.02 & 80.71 & 27.03 & 77.58 & 82.18 \\
Rating\% (\(\uparrow\))     & -     & 87.28 & 86.15 & 82.56 & 87.1  & 86.25 & 83.74 & 77.14 & 83.91 & 86.51 \\
Watermark Size (\(\downarrow\)) & -  & -     & 113   & 87    & 847   & >1024 & >1024 & 80 & 572   & 94 \\
\bottomrule
\end{tabular}
\end{table*}



\begin{table*}[htbp]
\centering
\begin{tabular}{lccc}
\toprule
        attack & CS+KGW & EXP & KGW \\  
        \midrule
        None & 96.5 & 89.5 & 179.0 \\  
        ContractionAttack & 87.5 & 93.0 & 167.0 \\  
        LowercaseAttack & 126.5 & 115.0 & 216.0 \\  
        MisspellingAttack\_(0.25,) & 90.5 & 101.0 & 193.0 \\  
        MisspellingAttack\_(0.5,) & 123.0 & 148.5 & 211.0 \\  
        SwapAttack\_0.05\_0.05\_0\_0 & 104.5 & 91.0 & 160.0 \\  
        SwapAttack\_0\_0\_0.05\_0 & 97.0 & 90.5 & 154.0 \\  
        SwapAttack\_0\_0\_0.1\_0 & 89.0 & 90.5 & 154.0 \\  
        SynonymAttack\_0.25 & 90.5 & 99.5 & 175.0 \\  
        SynonymAttack\_0.5 & 106.0 & 110.5 & 206.5 \\  
        SynonymAttack\_0.75 & 117.5 & 138.0 & 271.0 \\  
        SynonymAttack\_1 & 143.5 & 192.0 & 300.5 \\  
        TranslationAttack\_French & 130.0 & 135.0 & 216.0 \\  
        TranslationAttack\_Russian & 163.5 & 167.5 & 257.5 \\  
        TypoAttack\_(0.05,)" & 179.5 & 239.5 & 350.0 \\  
        TypoAttack\_(0.1,)" & 207.0 & 466.0 & 557.5 \\  
        ParaphraseAttack\_GPT3.5 & 197.0 & 412.0 & 1024.0 \\  
\bottomrule
\end{tabular}
\caption{Comparison of effiency for different generators and attacks.}
\label{tab:my_label}
\end{table*}
